The Art of Prompting: Event Detection based on Type Specific Prompts

We compare various forms of prompts to represent event types and develop a unified framework to incorporate the event type specific prompts for supervised, few-shot, and zero-shot event detection. The experimental results demonstrate that a well-defined and comprehensive event type prompt can significantly improve the performance of event detection, especially when the annotated data is scarce (few-shot event detection) or not available (zero-shot event detection). By leveraging the semantics of event types, our unified framework shows up to 24.3\% F-score gain over the previous state-of-the-art baselines.

==> Event Detection based on Type Specific Prompts/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Event detection~\cite{grishman1997information,chinchor1998muc,ahn2006stages} is the task of identifying and typing event mentions from natural language text. Supervised approaches, especially deep neural networks~\cite{chen-etal-2020-reading, xinyaduEMNLP2020,yinglinACL2020, jianliu2020emnlp, EEMQA_li, Lyu-etal-2021-zero}, have shown remarkable performance under a critical prerequisite of a large amount of manual annotations. However, they cannot be effectively generalized to new languages, domains or types, especially when the annotations are not enough~\cite{huang2016liberal,huang2020semi,extensively_lai_2020, Adaptive_Shirong_2021} or there is no annotations available \cite{Lyu-etal-2021-zero, zhang-etal-2021-zero, pasupat2014zero}.


\begin{table}[h]
\centering
\small
\begin{tabular}{S|Q}
\toprule
%     {\textbf{Event Rep}} &  Example\\ 
% \midrule
    Type Name & Attack\\
\midrule
    \multirow{2}{*}{Definition}      & Violent or physical act causing harm \\& or damage\\
\midrule
    Seed Trigger    & Invaded, airstrikes, overthrew, ambushed\\
\midrule
    Type Structure       & Attack, Attacker, Instrument, Victim, Target, Place\\
\midrule
   APEX Prompt       &  Attack, invaded airstrikes overthrew ambushed, an Attacker physically attacks a Target with Instrument at a Place \\%\sijia{OR: Attack events are usually triggered by phrases like \textit{invaded, airstrikes, overthrew, or ambushed}, meaning an Attacker physically attacks a Target with Instrument at a Place} \\
\bottomrule
\end{tabular}
\caption{Example of various forms prompt for the event type \textit{Conflict: Attack}}
\label{tab:attack_example}
\end{table}
Recent studies have shown that both the accuracy and generalizability of event detection can be improved via leveraging the semantics of event types based on various forms of prompts, such as event type specific queries~\cite{Lyu-etal-2021-zero, xinyaduEMNLP2020, jianliu2020emnlp}, definitions~\cite{chen-etal-2020-reading}, structures~\cite{yinglinACL2020, 10.1145/3308558.3313562}, or a few prototype event triggers~\cite{ wang2009character,Dalvi2012WebSetsES,pasupat2014zero,bronstein2015seed, lai2019extending, zhang-etal-2021-zero, Cong2021FewShotED}.
% , the approaches can be further improved and better transferred to new event types. 
Table \ref{tab:attack_example} shows an example of each form of event type prompt for detecting event mentions from the input sentence. These studies further encourage us to take another step forward and think about the following three questions: (1) does the choice of prompt matter when the training data is abundant or scarce? (2) what's the best form of prompt for event detection? (3) how to best leverage the prompt to detect event mentions? %\lifu{this motivation is not good enough. There could be two potential questions from reviewers: (1) have we really explored enough forms of prompts? e.g., questions, or parameters like p-tuning. (2) we can actually try similar frameworks for p-tuning and use sequence labeling for supervised event detection, but that framework cannot be applied to zero shot event detection -- Solution: (1) add a prompt that is based on event type specific question; (2) try p-tuning + sequence labeling for supervised event extraction}

To answer the above research questions, we conduct extensive experiments with various forms of prompts for each event type, including (a) \textit{event type name}, (b) \textit{prototype seed triggers}, (c) \textit{definition}, (d) \textit{event type structure} based on both event type name and its predefined argument roles, (e) free parameter based \textit{continuous soft prompt}, and (f) a more comprehensive event type description (named \textit{APEX prompt}) that covers all the information of prompts (a)-(d), under the settings of supervised event detection, few-shot and zero-shot event detection. We observe that (1) by considering the semantics of event types with most forms of prompts, especially seed triggers and the comprehensive event type descriptions, the performance of event detection under all settings can be significantly improved; (2) Among all forms of event representations, the comprehensive description based prompts show to be the most effective, especially for few-shot and zero-shot event detection; (3) Different forms of event type representations provide complementary improvements, indicating that they capture distinct aspects and knowledge of the event types.
%Each representation type is specialized in detecting regarding distinct aspects of event type.

In summary, our work makes the following contributions: 
\begin{itemize}[noitemsep,nolistsep,wide]
\item{we investigate various forms of prompts to represent event types for both supervised and weakly supervised event detection, and prove that a well-defined and comprehensive event type prompt can dramatically improve the performance of event detection and the transferability from old types to new types.}
\item{we developed a unified framework to leverage the semantics of event types with prompts for supervised, few-shot and zero-shot event detection, and demonstrate state-of-the-art performance with up to 24.3\% F-score improvement over the strong baseline methods.}
%\item{\lifu{we demonstrate state-of-the-art performance on supervised event detection, few-shot and zero-shot event detection}.}
\end{itemize}   




% Event extraction
%Event extraction~\cite{grishman1997information,chinchor1998muc,ahn2006stages} is a task to identify and type event mentions from natural language text. 

% \sijia{Why cares FSL and ZSL, why the design of prompt matters for zero and few shot learning}
%Supervised approaches show remarkable performance in many tasks across various fields and domains, under a critical prerequisite of a large amount of annotated training data. However, the lack of annotated data for event extraction discourage the development of effective models. The situation is more server for FSL and ZSL, causing either inadequate evaluation \cite{huang2017zero} or inefficient knowledge transfer ability. 

% prompt learning
%Prompt learning has been widely explored for general task such as summarization \cite{}, sentiment analysis, and machine translation. 

% \sijia{ some people believe that prompt does not matter}
%\cite{Raffel2020ExploringTL} argue that the choice of prompt doesn't matter when given abundant training data. 
%A task specific prompt suffice.
% \sijia{ when prompt matters (in related field)}
%However, for a more query-sensitive task such as QA, templates \sijia{cite} are commonly used to generate questions, and the design of the templates normally affect the performance. To fully leverage the knowledge in pre-trained language models, event queries or prompts must be delicately designed to be effective for zero-shot and few-shot learning.


% \sijia{Previous Approaches}
%Existing work represent event type with seed mentions, definitions, or predefined templates.  
%Additional seed examples can substantially improve system performance \cite{ wang2009character,  Dalvi2012WebSetsES,pasupat2014zero,bronstein2015seed, lai2019extending, zhang-etal-2021-zero, Cong2021FewShotED}.
%Graph knowledge structured with arguments and triggers mostly relies on sophisticate inferences module \cite{yinglinACL2020} or structured neural networks such as graph convolutional networks \cite{10.1145/3308558.3313562}.
%Predefined questions are commonly used in  question answering (QA)-based approaches \cite{Lyu-etal-2021-zero, xinyaduEMNLP2020, jianliu2020emnlp}. \sijia{one sentence conclude shortage of those approaches}

% Our claim is that the choice of prompt still matters.
%We conduct extensive experiments on different choices of prompt, aiming to prove that, for trigger event extraction with full supervision or limited amount of supervision, a well-defined prompt can greatly boost the performance.  

% The overall contributions of our work are:
% \begin{itemize}[noitemsep,nolistsep,wide]
% \item{We investigate exhaustive aspects to represent event type information. \sijia{diversity?}}
% \item{We conduct extensive experiments and prove that a well-defined event type prompt improve the performance for supervised learning, few-shot learning, and zero-shot learning.}
% \end{itemize}
% \newpage

==> Event Detection based on Type Specific Prompts/2_related_work.tex <==
\section{Related Work}

\label{sec:related_work}

% \lifu{condense each of the following subsections}

% Few-shot learning and Zero-shot learning learn effective latent linguistic features without large-scale data. Previous studies explore the alignment between unseen classes and seen classes.
% % Due to the development of large-scale pre-trained language models, prompting-based methods thrive. 
% % The substantial amount of encoded information 
% Prompting-based methods can potentially remove the complexities from matching the intrinsic semantic relatedness between unseen and seen classes. In this section, we review previous learning strategies for few-shot and zero-shot learning, and prompt learning applications.

%\lifu{add a paragraph about supervised event detection}

\paragraph{Supervised Event Detection:}
Most of the existing Event Detection studies follow a supervised learning paradigm~\cite{ji2008refining,liao2010using,mcclosky2011event,qiliACl2013,chen2015event,cao-etal-2015-improving,feng-etal-2016-language,yang-mitchell-2016-joint,nguyen_jrnn_2016,zhang2017improving,yinglinACL2020,cleve}, however, they cannot be directly applied to detect new types of events. Recently studies have shown that, by leveraging the semantics of event types based on type-specific questions~\cite{xinyaduEMNLP2020, jianliu2020emnlp, EEMQA_li, Lyu-etal-2021-zero} or seed event triggers~\cite{bronstein2015seed,lai2019extending, wang2021query}, the event detection performance can be improved. However, it's still unknown that whether they are the best choices of representing the semantics of event types.
%Question answering based event detection  approaches~\cite{xinyaduEMNLP2020, jianliu2020emnlp, EEMQA_li, Lyu-etal-2021-zero} can take advantage of the semantics of event types and the large-scale question answering datasets. 
%Query based approaches \cite{wang2021query} further emphasize the correlation between the event type and context semantics.
%Several studies have explored the semantics of event types based on seed event triggers~\cite{bronstein2015seed,lai2019extending, wang2021query}. Yet the other event representation forms are not fully explored.

 

\paragraph{Few-shot Event Detection:} Two primary learning strategies in few-shot classification tasks are Meta-Learning~\cite{Kang_ICCV_2019, Li2021BeyondMC, Xiao2020FewShotOD, Yan2019MetaRT, Chowdhury2021FewshotIC}, and Metric Learning~\cite{Sun2021FSCEFO, wang2020few, Zhang2021PNPDetEF, agarwal2021attention}. Several studies have exploited metric learning to align the semantics of candidate events with few examples of the novel event types for few-shot event detection~\cite{Exploiting_Lai_2020, Meta_Deng_2020, extensively_lai_2020, Cong2021FewShotED, honey_chen_2021,Adaptive_Shirong_2021}. However, due to the limited annotated data and the diverse semantics of event mentions, it's hard to design a metric distance to accurately capture the semantic similarity between the seed mentions and new ones.

\paragraph{Zero-shot Event Detection:} The core idea of zero-shot learning is to learn a mapping function between seen classes and their corresponding samples, and then apply it to ground new samples to unseen classes.~\newcite{huang2017zero} first exploited zero-shot event extraction by leveraging Abstract Meaning Representation~\cite{banarescu-etal-2013-amr} to represent event mentions and types into a shared semantic space. Recent studies~\cite{zhang-etal-2021-zero,Lyu-etal-2021-zero} further demonstrate that without using any training data, by leveraging large external corpus with abundant anchor triggers, zero-shot event detection can also be achieved with decent performance. However, such approaches cannot properly identify event mentions, i.e., distinguishing event mentions from none-event tokens.
%\sijia{However, such approaches rely on an independent trigger identification module to first identify the trigger candidates. Previous work show that trigger identification dominate the errors in event detection. Therefore, the unannotated data contains the knowledge to distinguish between event classes, but cannot help identify trigger candidates. }
%\lifu{dont understand. Re-write} 

\paragraph{Prompt Learning} Prompt learning aims to learn a task-specific prompt while keeping most of the parameters of the model freezed~\cite{Li2021PrefixTuningOC, hambardzumyan-etal-2021-warp, gpt3}. It has shown competitive performance in a wide variety of applications in natural language processing~\cite{Raffel2020ExploringTL, gpt3, autoprompt_emnlp20, Jiang2020HowCW, Lester2021ThePO, Schick2021naacl}. Previous work either use a manual \cite{petroni-etal-2019-language, gpt3, Schick_emnlp2021_few} or automated approach \cite{Jiang2020HowCW,yuan2021bartscore,Li2021PrefixTuningOC} to create prompts. In this work, we compare various forms of template based and free-parameter based prompts for event detection task under both supervised and weakly supervised setting.
%Automated learned templates includes \textit{discrete prompts} \cite{jiang2020know, yuan2021bartscore} and \textit{continuous prompt} \cite{Li2021PrefixTuningOC}.
%Continuous prompt are not suitable for FSL and ZSL, even initialize with well-defined prompt vector, because we don't have the annotated data to fine-tune the continuous prompt for novel classes.\lifu{rewrite this paragraph}

% ~\newcite{Adaptive_Shirong_2021} explored FrameNet to enrich the semantics of event
% Some approaches tries to enrich the event semantics.
% High-quality event semantic knowledge are usually introduced from external resources, such as FrameNet  \cite{Adaptive_Shirong_2021}. 
% % External resources can be considered to build knowledge prior distribution for event types \cite{Adaptive_Shirong_2021}. 
% However, due to the intrinsic difficulties of the event extraction task and the subtle difference in annotation strategies among event extraction tasks \cite{aguilar-etal-2014-comparison}, it's hard to align the external resources to the event type definitions. 


% \subsection{Few Shot}
% \label{sec:related_work_few}

% % \paragraph{Few-shot in CV}
% Two primary learning strategies in Few-shot image
% classification are Meta-Learning
% \cite{Kang_ICCV_2019, Li2021BeyondMC, Xiao2020FewShotOD, Yan2019MetaRT, Chowdhury2021FewshotIC}, 
% and Metric Learning \cite{Sun2021FSCEFO, wang2020few, Zhang2021PNPDetEF, agarwal2021attention}. Previous benchmark experiments \cite{Wang_meta_2019_ICCV} showed that metric learners usually outperform meta-learners in adapting to unseen data types. However, \cite{agarwal2021attention} pointed out that attention-based model can address problems like \textit{class confusion} and \textit{Catastrophic forgetting}. 


% \paragraph{Few-shot for Event Extraction}

% Metric learning has also been exploited by matching information between the examples for event extraction \cite{Exploiting_Lai_2020, Meta_Deng_2020, extensively_lai_2020, Cong2021FewShotED, honey_chen_2021}. However, due to the limited amount of annotated data and the semantics diversity of event mentions, it's hard to design a metric distance formula that captures a general relation between the seen mentions and other novel mentions.


% Some approaches tries to enrich the event semantics.
% High-quality event semantic knowledge are usually introduced from external resources, such as FrameNet  \cite{Adaptive_Shirong_2021}. 
% % External resources can be considered to build knowledge prior distribution for event types \cite{Adaptive_Shirong_2021}. 
% However, due to the intrinsic difficulties of the event extraction task and the subtle difference in annotation strategies among event extraction tasks \cite{aguilar-etal-2014-comparison}, it's hard to align the external resources to the event type definitions. 




% ===========================================================================

% \subsection{Zero Shot}
% \label{sec:related_work_zero}


% Existing work for Zero-shot in Computer Vision mostly explore the intrinsic semantic relatedness between seen and unseen classes.
% Unseen classes are classified by the metric distance \cite{Han2021ContrastiveEF, li2021attributemodulated} to seen classes in the embedding space. Such methods
% usually have a large bias towards seen classes, since the embedding is learned only on seen classes instances.
% attention-based ZSL methods:
% \cite{Xie_Attentive_cvpr_2019, Zhu_semantic_nips_2019, xu2020attribute, Liu2021GoalOrientedGE, chen2021transzero}
% utilize attribute descriptions as guidance to discover the more
% discriminative region (or part) features.

% For Zero-shot in Event Extraction, existing work \cite{zhang-etal-2021-zero, Lyu-etal-2021-zero} leverage anchor sentences from external corpus  and claim that they do not need any training data for ZSL. Such approaches greedily take advantage of the evaluation metrics (Hit@1, Hit@3, and Hit@5) following previous work \cite{huang2017zero}. Given considerably large external corpus with abundant anchor sentences, the event trigger are easier to be detected, especially for event classification task (when the trigger candidate/span is given).
% However, the subsequent result of relying on anchor triggers from un-annotated corpus is the difficult in distinguish between real event triggers and plain words that does not indicate any events. In other words, such approaches does not help trigger identification. 


% ===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.85\textwidth]{architecture2.pdf}
  \caption{Overview of the unified framework for event detection based on event type specific prompts.}
  \label{fig:architecture}
\end{figure*}
% \subsection{Prompt Learning}
% Prompt learning has been widely explored for general task such as summarization \cite{}, sentiment analysis, and machine translation.
% To leverage information and knowledge within pre-trained language models under limited budget, a task specific prompt is introduced to explicitly denote the problem to solve.
% By defining a novel prompt, a model pre-trained on base classes is able to adapt to new scenarios with few or no labeled data.

% Prompt engineering aims at creating a prompt that have the most effective performance. Previous work either take a manual \cite{petroni-etal-2019-language, NEURIPS2020_1457c0d6, Schick_emnlp2021_few} or automated approach \cite{jiang2020know} to create prompts. 
% Automated learned templates includes \textit{discrete prompts} \cite{jiang2020know, yuan2021bartscore} and \textit{continuous prompt} \cite{Li2021PrefixTuningOC}.
% Continuous prompt are not suitable for FSL and ZSL, even initialize with well-defined prompt vector, because we don't have the annotated data to fine-tune the continuous prompt for novel classes. 



==> Event Detection based on Type Specific Prompts/3_model.tex <==

\section{Problem Formulation}
\label{sec:model}
In this work, we aim to compare various forms of prompts to represent the event types under different settings, including supervised event detection, few-shot event detection and zero-shot event detection. Here, we first provide a definition for each setting of the event detection task and then describe the various forms of event type prompts.

\subsection{Settings of Event Detection}

\paragraph{Supervised Event Detection} We follow the conventional supervised event detection setting where both the training, validation and evaluation data sets cover the same set of event types. The goal is to learn a model $f$ on the training data set and evaluate its capability on correctly identifying and classifying event mentions for the target event types.

\paragraph{Few-shot Event Detection} There are two separate training data sets for few-shot event detection: (1) A large-scale base training data set $\mathcal{D}_{base}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{M}$ that covers the old event types (named \textit{base types}) with abundant annotations and $M$ denotes the number of base event types; (2) a smaller training data set $\mathcal{D}_{novel}=\{(\mathbf{x}_j, \mathbf{y}_j)\}_{j=1}^{N\times K}$ that covers $N$ novel event types, with $K$ examples each. Note that the base and novel event types are disjoint except the \texttt{Other} class. The model $f$ will be first optimized on $\mathcal{D}_{base}$, and then further fine-tuned on $D_{novel}$. The validation data set contains the mentions of both base and novel event types, while the evaluation data set only includes mentions of novel event types. The goal is to evaluate the generalizability and transferability of the model from base event types to new event types with few annotations.

\paragraph{Zero-shot Event Detection} The only difference between zero-shot and few-shot event detection lies in the training data sets. In zero-shot event detection, there is only a large-scale base training data set $\mathcal{D}_{base}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{M}$ with sufficient annotations for the base event types. The model $f$ will be only optimized on base event types and evaluated on the novel types, which is to measure the transferability of the model under a more challenging setting.

% In Zero-shot learning, we are given a training dataset $\mathcal{D}_{base}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{M}$ annotated with $C_{base}$ seen classes, and a novel dataset $\mathcal{D}_{novel}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{N}$ with $C_{novel}$ unseen classes. Note that annotation on base training set is disjoint with the novel set except the \texttt{Other} class, i.e., $C_{base} \cap C_{novel} = \{``O"\}$. 

% \subsection{Problem Definition}
% \paragraph{Few-shot Learning}
% We define a metric learning based few-shot training strategy as in \cite{majee2021fewshot} which
% proceeds in two stages: base training and few-shot adaptation. 
% A large-scale base training data set $\mathcal{D}_{base}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{M}$, and a novel dataset $\mathcal{D}_{novel}=\{(\mathbf{x}_j, \mathbf{y}_j)\}_{j=1}^{N\times K}$ are given, where $N$ is the novel classes, with $K$ examples each. During base training, a learner  $f$ learns to detect objects from base classes ($C_{base}$) using $\mathcal{D}_{base}$. 
% In the few-shot adaptation stage, $f$ is fine-tuned using instances in $D_{novel}$ consisting of classes $C_{base}\cup C_{novel}$ with only $K$ instances from N classes, such that $|C_{base} \cup  C_{novel}| = N$. The goal is to boost performance on novel classes in $D_{novel}$ with minimal degradation in performance of classes in $D_{base}$.
% % https://www.borealisai.com/en/blog/tutorial-2-few-shot-learning-and-meta-learning-i/
% % https://github.com/laiviet/ed-fsl-extensive-matching/blob/master/train.py

% \paragraph{Zero-shot Learning}
% In Zero-shot learning, we are given a training dataset $\mathcal{D}_{base}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{M}$ annotated with $C_{base}$ seen classes, and a novel dataset $\mathcal{D}_{novel}=\{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{N}$ with $C_{novel}$ unseen classes. Note that annotation on base training set is disjoint with the novel set except the \texttt{Other} class, i.e., $C_{base} \cap C_{novel} = \{``O"\}$. 


\subsection{Event Type Prompts}
We compare the following five forms of prompts to represent the event types:  %\lifu{need to state where are the prompts from, manually defined or extracted from anywhere}

% We extract three kinds of event representations from \cite{ldc_ace05}, specifically, event type name, definition, and event structure, and two statistical prompt seed trigger and seed mention from the training data, and an extra type of comprehensive event prompt incorporating the above representations. 
% % event representation
% Each event type prompt will be represented with a natural language sequence of words, denoted as $T= \{\tau_1^t, \tau_2^t, \dots, \tau_K^t\}$, for event type $t$. 

\paragraph{Event Type Name} The most straightforward and intuitive representation of an event type is the type name, which usually consists of one to three tokens. As the most basic and discriminative representations of event types, we include them in all the following text-based event type prompts.%\lifu{confirm, it's not included in soft prompt} \sijia{yes}

%. Type name is the most indicative words to represent the event category, mostly in two to three tokens. Due to the discriminative ability of event type name, we include them in every corresponding event type prompt.


\paragraph{Definition} The type name sometimes cannot accurately represent the semantics of an event type due to the ambiguity of the type name as well as the variety of the event mentions. For example, \textit{execute} can either refer to \textit{putting a legal punishment into action} or \textit{performing a skillful action or movement}. 
%\lifu{just channge to another example, e.g., execute, sentence, all these are ambiguous -- I'm saying, create an example similar to Meet, which has multiple meanings so simply using the event type name is not enough} \sijia{a \textit{Conflict:Arrest-Jail} event takes place whenever a state actor take custody or constrain the movement of a person,  or a person serve a sentence.} 
The definitions instead formally describe the meaning of the event types. Taking the event type \textit{Attack} from ACE as an example, its definition is \textit{violent or physical act causing harm or damage}

% =================================
% From ACL
\paragraph{Prototype Seed Triggers} Seed trigger based representation consists of the type name and a list of prototype triggers. Given an event type $t$ and its annotated triggers, following~\cite{wang2021query}, we select the top-$K$\footnote{In our experiments, we set $K=4$.} ranked words as the prototype triggers based on the probability $f_t/f_o$ of each word, where $f_o$ is the frequency of the word from the whole training dataset and $f_t$ is the frequency of the word being tagged as an event trigger of type $t$. Thus, for the event type \textit{Attack}, we represent it as \textit{attack invaded airstrikes overthrew ambushed}. 

% For each event type $t$, we collect a set of annotated triggers from the training examples. For each unique trigger word, we compute its frequency from the whole training dataset as $f_o$ and its frequency of being tagged as an event trigger of type $t$ as $f_t$, and then obtain a probability $f_t/f_o$, which will be used to sort all the annotated triggers for event type $t$. We select the top-$K$\footnote{In our experiments, we set $K=4$.} ranked words as triggers prompt. Taking the event type \textit{Attack} from ACE as an example, we represent it as \textit{Attack [SEP] invaded airstrikes overthrew ambushed}.
% From ACL
% =================================

% \paragraph{Seed Mention}
%In addition to seed trigger, we also explore the semantics of trigger token within context. To achieve that, we concatenate the entire seed sentences, and take the encoding of the annotated trigger as the prompt. 

\paragraph{Event Type Structure} Each event is associated with several arguments, indicating the core participants. Our preliminary experiment shows that for certain event types, the arguments can help determine the existence of its corresponding events. For example, given a sentence, if no person presents in the context, there should be no \textit{Meet} events. Given that, we define an event type structure, which consists of the event type name and argument roles, to represent the event type, e.g., \textit{attack attacker victim target instrument place} for \textit{Attack}.

% , for example, the event \texttt{Attack} is associated with \texttt{victim}, \texttt{attacker}, \texttt{place}. Our preliminary experiment shows that for certain event types, the argument extraction result can help filtering false positive trigger predication. For example, for \textit{Contact:Meet} event, if no person are detected during argument detection stage, then the detected trigger is probably a false positive prediction. Therefore, we believe that argument will help identify the trigger to some extend. 

\paragraph{Continuous Soft Prompt} Inspired by the recent success of prompt tuning methods in various NLP applications, we also adopt a continuous soft prompt, i.e., a free vector of parameter, to represent each event type. More details regarding the learning of soft prompts are described in Section~\ref{sec:unified_ed}.

\paragraph{APEX Prompt} We assume a better representation of an event type should cover the important information of all the above prompts. Thus we define a more comprehensive description (named \textit{APEX prompt}) for each event type by concatenating its event type name, seed triggers, and definition which covers all the argument roles. For example, The APEX prompt for \textit{Attack} event type is \textit{attack, invaded airstrikes overthrew ambushed, an attacker physically attacks a target with an instrument at a place}.

In our experiments, the event type names and event type structures are automatically extracted from the target event ontology, such as ACE~\cite{ldc_ace05}, ERE~\cite{song2015light} and MAVEN~\cite{MAVEN}. The prototype seed triggers for each event type are automatically selected from its annotated data. The definitions and APEX prompts are based on the official annotation guides for each target event ontology~\cite{ldc_ace05,song2015light,MAVEN} and the available definitions in FrameNet~\cite{baker1998berkeley} with manual editing.

%\sijia{event type name, definition, prototype seed triggers, event structure, continuous soft prompt and APEX prompt. The type name, and event structure are extracted from the released guideline \cite{ldc_ace05, song2015light, MAVEN}. Prototype seed triggers can be statistically extracted from the training data. We manually rewrite the definition and APEX prompts as concise sentences. And soft prompts are randomly initialized.}

%The above types of event representation explicitly express different aspects of the event semantics. A comprehensive APEX prompt is a representation that jointly leverage all of them. It starts with event type name and seed trigger, followed by a rephrased definition. The rephrased definition is based on the event definition and it must contains all of its arguments. For \textit{Attack}, we construct the comprehensive prompt as \textit{Attack-[SEP]-invaded-airstrikes-overthrew-ambushed-[SEP]-An-Attacker-physically-attacks-a-Target-with-Instrument-at-a-Place.}

\section{A Unified Framework for Event Detection}
\label{sec:unified_ed}

%\lifu{the following description needs to be rewriten; cannot be the same as the ACL submission}

Figure~\ref{fig:architecture} shows the overview of our unified framework, which leverages event type specific prompts to detect events under supervised, few-shot and zero-shot settings. Next, we will describe the details of this framework.

\paragraph{Context Encoding} Given an input sentence $W = \{w_{1}, w_{2}, \dots, w_{N} \}$, we take each event type prompt $T= \{\tau_1^t, \tau_2^t, \dots, \tau_K^t\}$ as a query to extract the corresponding event triggers. Specifically, we first concatenate them into a sequence as follows:
\begin{align}
\small
\text{[CLS]} \; \tau_1^t\; ...\; \tau_K^t\;  \text{[SEP]} \; w_{1}\; ...\; w_{N}\; \text{[SEP]} \nonumber
\end{align}
where [SEP] is a separator from the BERT encoder~\cite{devlin-etal-2019-bert}. 
We use a pre-trained BERT encoder to encode the whole sequence and get contextual representations for the input sentence $\boldsymbol{W} = \{\boldsymbol{w}_0, \boldsymbol{w}_2, ..., \boldsymbol{w}_N\}$ as well as the event type prompt $ \boldsymbol{T} = \{\boldsymbol{\tau}_0^t, \boldsymbol{\tau}_1^t, ..., \boldsymbol{\tau}_K^t\}$.\footnote{We use bold symbols to denote vectors.}

\paragraph{Event Type Aware Contextual Representation} Given a prompt of each event type, we aim to  extract corresponding event triggers from the input sentence automatically. To achieve this goal, we need to capture the semantic correlation of each input token to the event type. Thus we apply attention mechanism to learn a weight distribution over the sequence of contextual representations of the event type query for each token:
\begin{align}
\small
    & \boldsymbol{A}_{i}^{T} = \sum_{j=1}^{|T|}\alpha_{ij}\cdot\boldsymbol{T}_j,\,\, \textrm{where}\,\,\alpha_{ij} = \cos(\boldsymbol{w}_i,\ \boldsymbol{T}_j),\nonumber
\end{align}
where $\boldsymbol{T}_j$ is the contextual representation of the $j$-th token in the sequence $T= \{t, \tau_1^t, \tau_2^t, \dots, \tau_K^t\}$. $\cos(\cdot)$ is the cosine similarity function between two vectors. $\boldsymbol{A}_{i}^{T}$ denotes the event type $t$ aware contextual representation of token $w_i$.


\paragraph{Event Detection} With the aforementioned event type prompt attention, each token $w_i$ from the input sentence will obtain a enriched contextual representations $\boldsymbol{A}_{i}^{T}$. We concatenate them with the original contextual representation $\boldsymbol{w}_i$ from the encoder, and classify it into a binary label, indicating it as a candidate trigger of event type $t$ or not:
\begin{align*}
\small
  \boldsymbol{\tilde{y}}_i^t = \boldsymbol{U}_{o}([\boldsymbol{w}_i;\  \boldsymbol{A}_{i}^{T}; \boldsymbol{P}_i]) \;,
\end{align*}
where $[;]$ denotes concatenation operation, $\boldsymbol{U}_{o}$ is a learnable parameter matrix for event trigger detection, and $\boldsymbol{P}_i$ is the one-hot part-of-speech (POS) encoding of word $w_i$. 

For continuous soft prompt based event detection, we follow~\newcite{Li2021PrefixTuningOC} where a prefix index $q$ is prepended to the input sequence $W' = [q;\; W]$. The prefix embedding is learned by $\boldsymbol q=\text{MLP}_\theta(\boldsymbol Q_\theta[q])$, where $\boldsymbol Q_\theta\in \mathbb{R}^{|\mathcal Q|\times k}$ denotes the embedding lookup table for the vocabulary of prefix indices. Both $\text{MLP}_\theta$ and $\boldsymbol Q_\theta$ are trainable parameters. After obtaining the prefix embedding $\boldsymbol q$, we concatenate it with the initialized token embeddings of the input sentence and feed them to BERT encoder. For each token $w_i$, we obtain its contextual representation $\boldsymbol w_i$, concatenate it with its POS tag encoding $\boldsymbol{P}_i$, and then classify the token into a binary label.

%We use $\mathcal Q$ to denote the vocabulary of prefix indices. The embeddings of the prefix indices are determined by a embedding matrix $\boldsymbol Q_\theta\in \mathbb{R}^{|\mathcal Q|\times k}$ and a reparameterized matrix $\text{MLP}_\theta(\cdot)$ that maps from dimension $k$ to $d$, where $d$ is the embedding dimension of the language model. So the prefix embeddings are obtained from $\boldsymbol q_i=MLP_\theta(Q_\theta[q_i,:])$, where $MLP_\theta(\cdot)$ and $Q_\theta$ are trainable parameters. \lifu{still don't understand how you learn the embeddings of Q and embddings of the sentence. add description how did you get the embedding for each token}\sijia{word embedding is not changed. Since Bert is a masked LM, the prefix only affect attentions in the following layers. Unlike in encoder-decoder LMs, the prefix will affect the encodings of the subsequent words} \lifu{what does $Q_\theta[q_i,:]$ mean}\sijia{its just a embedding layer, which takes in prefix indices like 0, 1, 2, and generate a embedding}
% \lifu{what does the following formula mean? what is h? why use two formulas? you need to connect it to the classification formula, pointing out which representation you used to do the classification}
% \sijia{So that the prefix embedding becomes
% $\boldsymbol q_i=MLP_\theta(Q_\theta[q_i,:])$. Both $MLP_\theta(\cdot)$ parameters and $Q_\theta$ parameters are trainable.}


%\sijia{Specifically, following \newcite{Li2021PrefixTuningOC}, a prefix $\boldsymbol p$ is prepended to the input sequence to obtain $\boldsymbol x' = [\boldsymbol p;\; \boldsymbol x]$. We use $|\boldsymbol P|$ to denote the length of all possible prefix indices. The embeddings of the prefix indices are given by a reparameterized matrix $MLP_\theta(\boldsymbol P_\theta)\in \mathbb{R}^{|P|\times d}$, where $d$ is the embedding dimension of the language model.}

\begin{table*}[h]
\centering
\small
\begin{tabular}{c|c|c|c|c|Q}
\toprule
\multicolumn{2}{c|}{Dataset} &  ACE05-E+ & ERE-EN & MAVEN & \multicolumn{1}{c}{Notes}
 \\
\midrule
\multirow{2}{*}{\# Types}&
{Base}  &  18 & 25    &120& - \\
&{Novel}  &  10 &  10   &45& - \\
\midrule
\multirow{2}{*}{\# Mentions}&
{ Base}  &  3572 & 5449    & 93675 & - \\
&{Novel} &  1724 & 3183    & 3201  & - \\
\midrule
\multirow{2}{*}{Train}
& Few-shot & 3216 & 3886  &88085 &    Include mentions of base types and a small set of mentions for novel types \\
% \cmidrule{2-6}
& Zero-shot & 3116  & 3786  & 87635 &   Include mentions of base types \\
\midrule
\multicolumn{2}{c|}{\multirow{2}{*}{Validation} }    & 900   & 2797   &3883&  Mentions of base and novel types \\
\multicolumn{2}{c|}{}                         & ( 51\%/49\% ) & ( 53\%/47\% ) & ( 71\%/23\% )& Indicate the base/novel mention ratio \\
\midrule
\multicolumn{2}{c|}{Evaluation}       & 1195        &  2012        &1652 & Include mentions of novel types\\
% \midrule
% \multirow{4}{*}{Dev}
% & train & 3116  & 3786  & 87635 &   mentions of base types \\
% \cmidrule{2-6}
% & { dev}     & 900   & 2797   & 3883 & mention of base and novel types \\
% &                           & ( 51\%/49\% ) & ( \%/\% ) &  ( 71\%/23\% )&   (base/novel mention ratio)\\
% \cmidrule{2-6}
% & test       & 1195        &  2012        &1652&  mentions of novel types\\
% & train & 3116      & 3786      & sent ONLY has \textbf{base}\\
% & dev   & 1295*50\% & 2112*50\% & sent ONLY has \textbf{novel} * 50\%\\
% & test  & 1295*50\% & 2112*50\% & sent ONLY has \textbf{novel} * 50\%\\
\bottomrule
\end{tabular}
\caption{Data statistics for ACE2005, ERE and MAVEN datasets under the few-shot and zero-shot event detection settings.}
\label{tab:data statistics}
\end{table*}


\paragraph{Learning Strategy}
% supervised learning
The learning strategy varies for supervised learning, few-shot learning and zero-shot learning. For supervised learning, we optimize the following objective for event trigger detection
\begin{align*}
\small
    \mathcal{L} = -\frac{1}{|\mathcal{T}||\mathcal{N}|}
        \sum_{t\in\mathcal{T}}
        \sum_{i=1}^{|\mathcal{N}|} \boldsymbol{y}_i^t\cdot\log \boldsymbol{\tilde{y}}_i^t\;,
\end{align*}
where $\mathcal{T}$ is the set of target event types and $\mathcal{N}$ is the set of tokens from the training dataset. $\boldsymbol{y}_i^t$ denotes the groundtruth label vector.

For few-shot event detection, we optimize the model on both base training data set and the smaller training data set for novel event types:
% {\small
\begin{align*}
    \small\mathcal{L} = &\small -\frac{1}{|\mathcal{T}^B||\mathcal{N}^B|}
        \sum_{t\in\mathcal{T}^B}
        \sum_{i=1}^{|\mathcal{N}^B|} \boldsymbol{y}_i^t\cdot\log \boldsymbol{\tilde{y}}_i^t\\
        & \small- \alpha\frac{1}{|\mathcal{T}^N||\mathcal{N}^N|}
        \sum_{t\in\mathcal{T}^N}
        \sum_{i=1}^{|\mathcal{N}^N|} \boldsymbol{y}_i^t\cdot\log \boldsymbol{\tilde{y}}_i^t
\end{align*}
% }%
where $\mathcal{T}^B$ and $\mathcal{N}^B$ denote the set of base event types and tokens from the base training data set, respectively. $\mathcal{T}^N$ is the set of novel event types. $\mathcal{N}^N$ is the set of tokens from the training data set for novel event types. $\alpha$ is a hyper-parameter to balance the two objectives.

For zero-shot event detection, as we only have the base training data set, we minimize the following objective: 
\begin{align*}
\small
    \mathcal{L} = -\frac{1}{|\mathcal{T}^B||\mathcal{N}^B|}
        \sum_{t\in\mathcal{T}^B}
        \sum_{i=1}^{|\mathcal{N}^B|} \boldsymbol{y}_i^t\cdot\log \boldsymbol{\tilde{y}}_i^t\;.
\end{align*}


==> Event Detection based on Type Specific Prompts/4_experiments.tex <==


\begin{table*}[h]
\centering
\small
\begin{tabular}{l|c|c|c}
\toprule
    \textbf{Method} &  Supervised ED & Few-shot ED & Zero-shot ED\\ 
\midrule
\multirow{2}{*}{State of the art} & 73.3 & 35.2$^*$ & $ 49.1^*$\\%53.5 [10/23] \\
& \cite{vannguyen2021crosstask} 
& \cite{extensively_lai_2020}
& \cite{zhang-etal-2021-zero} \\
\midrule
(a) Event Type name & 72.2  & 52.7  & 49.8\\
(b) Definition &73.1        & 46.7  & 45.5\\
(c) Seed Triggers &73.7	    & 53.8  & 52.4\\
    % Seed Mention & 73.2 &  &\\
(d) Event Type Structure &72.8 &50.4&48.0\\
(e) Continuous Soft Prompt & 68.1 & 48.2 & - \\
% \cmidrule{2-5}
\midrule
% \multirow{2}{2cm}{Prompt - Comprehensive} 
Majority Voting of (a)-(e)  & 73.9 & 52.1 & 48.7\\
\midrule
  %Fusion   & 74.3  & &\\
(f) \textbf{APEX Prompt} &\textbf{ 74.9 }& \textbf{57.4} &\textbf{55.3} \\
\bottomrule
\end{tabular}
\caption{Results of event detection (ED) on ACE05 (F1-score, \%) $^*$ indicates evaluation on our data set split. }
\label{tab:ACE}
\end{table*}


\begin{table*}[h]
\centering
\small
\begin{tabular}{l|c|c|c}
\toprule
    {\textbf{Method}} &  Supervised ED  & Few-shot ED & Zero-shot ED \\ 
\midrule
\multirow{2}{*}{State of the art} & 59.4 & 33.0$^*$ &  $41.2^*$\\%* \\
& \cite{text2event} 
& \cite{extensively_lai_2020}
& \cite{zhang-etal-2021-zero} \\
\midrule
    (a) Event Type Name & 58.2  & 44.8 & 40.5  \\
    (b) Definition      & 57.9  & 44.2 & 40.4  \\
    (c) Seed Triggers    & 60.4  & 50.4 & 49.8  \\
%    Seed Mention    & 57.2  &      &       \\
    (d) Event Type Structure       & 59.1  & 48.5 & 48.7   \\
    (e) Continuous Soft Prompt & 55.6& 41.7 & - \\
\midrule
    Majority Voting of (a)-(e)  &  60.2 & 47.9 & 48.3 \\
\midrule
    % Fusion &   & & \\
    (f) \textbf{APEX Prompt} &  \textbf{63.4}  & \textbf{52.6} & \textbf{49.9} \\
\bottomrule
\end{tabular}
\caption{Results of event detection (ED) on ERE (F1-score, \%). $^*$ indicates evaluation on our data set split.}
\label{tab:ERE}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{l|c|c|c}
\toprule
    {\textbf{Method}} &  Supervised & Few-shot & Zero-shot \\ 
\midrule
\multirow{2}{*}{State of the art} & 68.5 & 57.0 & 40.2* \\
& \cite{cleve} & \cite{honey_chen_2021}& \cite{zhang-etal-2021-zero}\\
\midrule
    (a) Event type name & 68.8 & 63.4  & 58.8 \\
    (b) Definition & 67.1 &  56.9 & 52.9\\
    (c) Seed Triggers & 68.7 & 65.1  & 62.2\\
    (e) Continuous Soft Prompt & 64.5 & 38.6 & - \\
\midrule
Majority Voting of (a)-(e) & 68.4 & 63.4 & 58.6 \\
\midrule
    (f) \textbf{APEX Prompt} & \textbf{68.8}  & \textbf{ 68.4} & \textbf{64.5} \\
\bottomrule
\end{tabular}
\caption{Results of event detection (ED) on MAVEN (F1-score, \%).  $^*$ indicates evaluation on our data set split.}
\vspace{-1.2em}
\label{tab:MAVEN}
\end{table*}


\section{Experiment Setup}
\label{sec:experiments}
\subsection{Datasets}

We perform experiments on three public benchmark datasets, include ACE05-E$^+$ (Automatic Content Extraction)\footnote{\url{https://catalog.ldc.upenn.edu/LDC2006T06}}, ERE (Entity Relation Event)~\cite{song2015light}\footnote{Following~\citet{yinglinACL2020}, we merge LDC2015E29, LDC2015E68, and LDC2015E78 as the ERE dataset.}, and MAVEN\cite{MAVEN}. On each dataset, we conduct experiments under three settings: supervised event detection, few-shot and zero-shot event detection. 

For supervised event detection, we use the same data split as the previous studies~\cite{qiliACl2013,wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020,yinglinACL2020,vannguyen2021crosstask, MAVEN} on all the three benchmark datasets.

For few-shot and zero-shot event detection on MAVEN, we follow the previous study~\cite{honey_chen_2021} and choose 120 event types with the most frequent mentions as the base event types and the rest 45 event types as novel ones. 
%We split the open-source training set and development set by base and novel types to evaluate the few-shot and zero-shot learning performance.
% \lifu{what does it mean? are the train, dev and test splits the same as the reference?}\sijia{The base/novel types split follows \cite{honey_chen_2021}, but not the train/test sentence split.  The statistics remains similar (similar train/dev/test ratio). I didn't use the released split in their github because I found the split flawed. see the comment below:
% for each event type, they only assign a small number of sentences to be test, for example:
% "Suspicion": [30655, 2288, 996, 30682, 2383, 631, 2361, 2302, 2374, 30666, 2344, 30222, 2355, 1711], where the numbers are sentence indices
% }\lifu{how did you re-split it? are you following the same process described in the last paragraph in this section?}\sijia{yes} 
For few-shot and zero-shot event detection on ACE and ERE, previous studies~\cite{extensively_lai_2020, Exploiting_Lai_2020, honey_chen_2021} follow different data splits and settings, making it hard for fair comparison. Considering the research goals of few-shot and zero-shot event detection, we define the following conditions to split the ACE and ERE datasets:
\begin{itemize}
    \item The base event types and novel event types should be disjoint except \texttt{Other}.
    \item Each base or novel event type should contain at least 15 instances.
    \item The training set should contain sufficient annotated event mentions.
\end{itemize}

To meet the above conditions, for ACE, we define the event types of 5 main event categories: \textit{Business}, \textit{Contact}, \textit{Conflict}, \textit{Justice} and \textit{Movement} as the base event types, and types of the remaining 3 main categories: \textit{Life}, \textit{Personnel} and \textit{Transaction} as the novel event types. In total, there are 18 qualified base types and 10 qualified novel types (the others do not satisfy the second condition). For ERE, we use the exact same 10 novel event types as ACE, and the rest 25 types as base event types. 

After defining the base and novel event types, we further create the training, validation and evaluation splits for all three datasets. For few-shot event detection, we use the sentences with only base event type mentions as the base training data set, and randomly select 10 sentences with novel event type mentions as the additional smaller training data set. We use the sentences with both base and novel event type mentions as the development set, and use the remaining sentences with only novel event type mentions as the evaluation dataset. For zero-shot event detection, we use the same development and evaluation set as few-shot event detection, and remove the instances with novel event mentions from the training set. For both zero-shot and few-shot event detection, we randomly split the sentences without any event annotations proportionally to the number of sentences with event mentions in each set. Table \ref{tab:data statistics} shows the detailed data statistics for all the three datasets under the few-shot and zero-shot event extraction settings.

% Automatic Content Extraction 2005 (ACE05-E$^+$)\footnote{\url{https://catalog.ldc.upenn.edu/LDC2006T06}} and Entity Relation Event (ERE-EN)~\cite{song2015light}\footnote{Following~\citet{yinglinACL2020}, we merge LDC2015E29, LDC2015E68, and LDC2015E78 as the ERE dataset.}, and MAVEN\cite{MAVEN}. We conducted experiment under three settings: supervised event detection, few-shot and zero-shot event detection. 

% To fully leverage the annotated data in the three datasets, we use different dataset split strategies for the three settings. For supervised event extraction, we use the same data split as~\cite{qiliACl2013,wadden-etal-2019-entity,yinglinACL2020,xinyaduEMNLP2020,yinglinACL2020,vannguyen2021crosstask, MAVEN}.
% For few-shot and zero-shot settings on the MAVEN dataset, we choose 120 event types with the most frequent mentions as base types and the rest 45 type as novel types following ~\cite{honey_chen_2021}. We split the open-source training set and development set by base and novel types to evaluate the few-shot and zero-shot learning performance.

% For few-shot and zero-shot settings on the ACE and ERE dataset, we create new splits.
% Previous work follows various \cite{extensively_lai_2020, Exploiting_Lai_2020, honey_chen_2021, MAVEN} training / evaluation event type split, however, due to the limited number of novel event instances given in the development and test set, the evaluation can be biased. Note that there are abundant novel event instances in the training set. Aiming to use them to create a finer evaluation set, we split the datasets to satisfy the following three conditions:
% \begin{itemize}
%     \item $C_{base}\cap C_{novel} = \{``O"\}$.
%     \item Each event subtypes should contain at least 15 instances.
%     \item The training set should contain sufficient annotated event instances.
% \end{itemize}
% Hence, for ACE dataset,  we define event subtypes of 5 main event types: \textit{Business}, \textit{Contact}, \textit{Conflict}, \textit{Justice} and \textit{Movement} as base event types, and subtypes of the remaining 3 a main types, \textit{Life}, \textit{Personnel} and \textit{Transaction} as novel event types. There are 18 qualified base subtypes and 10 qualified novel subtypes (the rest subtypes does not satisfy the second condition). For ERE dataset, we use the exact same 10 novel event subtypes from 3 main types (\textit{Life}, \textit{Personnel} and \textit{Transaction}), and the rest 25 subtypes from the 6 main types as base subtypes. (In the remaining sections, we will use event type to denote subtype.)

% The dataset splits are different between few-show and zero-shot setting, because a limited amount of novel instances are given to few-shot learning. For few-shot learning, we put sentences with only base events in the training dataset and ten random novel instances and the rest sentences with only novel events in the test dataset. To address \textit{Catastrophic forgetting}, we keep sentences with both base events and novel events in the development set. Sentences without event mentions are split based on event occurrence proportion. 
% For zero-shot learning, we keep sentences with only base events in the training dataset and randomly split sentences with only novel events in the development and test dataset. Similarly, we randomly split sentences without event mentions based on event occurrence proportion. Table \ref{tab:data statistics} shows the details of data statistics for ACE and ERE datasets.


\subsection{Hyperparameters and Evaluation}
For a fair comparison with the previous baseline approaches, we use the same pre-trained \texttt{bert-large-uncased} model for fine-tuning and optimizing our model with BertAdam. For supervised event detection, we optimize the parameters with grid search: training epoch 3, learning rate $\in [3e\text{-}6, 1e\text{-}4]$, training batch size $\in\{8, 12, 16, 24, 32\}$, dropout rate $\in\{0.4, 0.5, 0.6\}$. The running time is up to 3 hours on one Quadro RTX 8000. For evaluation, we use the same criteria as previous studies~\cite{qiliACl2013,chen2015event,nguyen_jrnn_2016,yinglinACL2020}: an event mention is correct if its span and event type matches a reference event mention. %Each candidate may act as a trigger for multiple event occurrences.


% ACE:
% Base:
%     Business:Declare-Bankruptcy: 43
%     Business:Start-Org: 47
%     Business:End-Org: 37
%     Conflict:Attack: 1537
%     Contact:Meet: 279
%     Contact:Phone-Write: 123
%     Conflict:Demonstrate: 81
%     Justice:Sue: 76
%     Justice:Arrest-Jail: 88
%     Justice:Execute: 21
%     Justice:Trial-Hearing: 109
%     Justice:Sentence: 99
%     Justice:Charge-Indict: 106
%     Justice:Convict: 76
%     Justice:Release-Parole: 47
%     Justice:Fine: 28
%     Justice:Appeal: 43
%     Movement:Transport: 718
% Novel:
%     Personnel:Elect: 182
%     Personnel:Start-Position: 117
%     Personnel:End-Position: 200
%     Life:Injure: 137
%     Life:Die: 594
%     Life:Be-Born: 50
%     Life:Divorce: 29
%     Life:Marry: 83
%     Transaction:Transfer-Money: 194
%     Transaction:Transfer-Ownership: 126
% filtered types: 
%     {'Justice:Acquit': 6, 'Justice:Pardon': 2, 'Justice:Extradite': 7, Personnel:Nominate: 12, Business:Merge-Org: 14}
% sums of main type: Conclusion403
%     {'Movement': 718, 'Personnel': 511, 'Conflict': 1618, 'Contact': 402, 
%      'Life': 893, 'Transaction': 320, 'Justice': 693, 'Business': 141}


% =================================
% ERE: 
% Base:
%     business:endorg: 39
%     business:mergeorg: 15
%     business:startorg: 45
%     conflict:attack: 1451
%     conflict:demonstrate: 112
%     contact:broadcast: 422
%     contact:contact: 672
%     contact:correspondence: 241
%     contact:meet: 330
%     justice:acquit: 24
%     justice:appeal: 13
%     justice:arrestjail: 170
%     justice:chargeindict: 140
%     justice:convict: 70
%     justice:execute: 68
%     justice:extradite: 26
%     justice:fine: 26
%     justice:pardon: 42
%     justice:releaseparole: 59
%     justice:sentence: 100
%     justice:sue: 48
%     justice:trialhearing: 138
%     movement:transportartifact: 92
%     movement:transportperson: 837
%     manufacture:artifact: 132
% Novel:
%     life:beborn: 76
%     life:die: 769
%     life:divorce: 32
%     life:injure: 118
%     life:marry: 80
%     personnel:elect: 132
%     personnel:endposition: 261
%     personnel:nominate: 39 X
%     personnel:startposition: 163
%     transaction:transaction: 126 X
%     transaction:transfermoney: 1009
%     transaction:transferownership: 573
% filtered type: 
%     {'business:declarebankruptcy': 5}
% sums of main type:
%     {'life': 1075, 'conflict': 1563, 'contact': 1665, 'transaction': 1708, 'movement': 929, 'personnel': 595, 'justice': 924, 'manufacture': 132, 'business': 104}

% MAVEN 
% Base: {'Not': 404429, 'Causation': 4229, 'Process_start': 4203, 'Catastrophe': 3975, 'Hostile_encounter': 3620,
%  'Attack': 3579, 'Competition': 3179, 'Motion': 2705, 'Social_event': 2098, 'Killing': 2036, 'Process_end': 1795,
%  'Conquering': 1785, 'Statement': 1722, 'Self_motion': 1668, 'Arriving': 1633, 'Destroying': 1478, 'Coming_to_be': 1419,
%  'Military_operation': 1312, 'Damaging': 1257, 'Bodily_harm': 1257, 'Death': 1227, 'Hold': 1197,
%  'Cause_change_of_strength': 1183, 'Creating': 1164, 'Cause_change_of_position_on_a_scale': 1150, 'Control': 1134,
%  'Earnings_and_losses': 1107, 'Becoming': 1089, 'Getting': 1083, 'Know': 1027, 'Arranging': 1017, 'Action': 986,
%  'Escaping': 965, 'Preventing_or_letting': 959, 'Change_of_leadership': 957, 'Defending': 938, 'Traveling': 937,
%  'Presence': 932, 'Change': 876, 'Motion_directional': 875, 'Placing': 852, 'Cause_to_be_included': 850,
%  'Participation': 850, 'Influence': 814, 'Judgment_communication': 768, 'Name_conferral': 763,
%  'Expressing_publicly': 756, 'Request': 751, 'Giving': 723, 'Removing': 687, 'Supporting': 680,
%  'Agree_or_refuse_to_act': 659, 'Recording': 656, 'Supply': 618, 'Using': 612, 'Use_firearm': 588, 'Communication': 586,
%  'Reporting': 583, 'Choosing': 581, 'Departing': 526, 'Bringing': 523, 'Sending': 513, 'Assistance': 468,
%  'Dispersal': 451, 'Cause_to_make_progress': 450, 'Building': 443, 'Deciding': 434, 'Come_together': 431,
%  'Perception_active': 428, 'Violence': 419, 'Manufacturing': 412, 'Cause_to_amalgamate': 383, 'Arrest': 379,
%  'Hindering': 373, 'Receiving': 362, 'Response': 356, 'Achieve': 348, 'Terrorism': 348, 'Aiming': 347,
%  'Recovering': 339, 'Change_event_time': 328, 'Expansion': 325, 'Scrutiny': 325, 'Besieging': 312, 'Check': 301,
%  'Publishing': 294, 'Becoming_a_member': 292, 'Criminal_investigation': 277, 'Openness': 274, 'Collaboration': 274,
%  'Committing_crime': 267, 'Being_in_operation': 264, 'Coming_to_believe': 256, 'Connect': 252, 'Surrendering': 246,
%  'Legal_rulings': 243, 'Sign_agreement': 236, 'Confronting_problem': 225, 'Preserving': 222, 'Temporary_stay': 221,
%  'Warning': 220, 'GiveUp': 217, 'Quarreling': 215, 'Convincing': 206, 'Change_sentiment': 201, 'Telling': 195,
%  'Protest': 186, 'Legality': 175, 'Testing': 163, 'Rescuing': 162, 'Commitment': 160, 'Resolve_problem': 160,
%  'Employment': 159, 'Emptying': 154, 'Commerce_sell': 153, 'Releasing': 143, 'Body_movement': 143,
%  'Expend_resource': 137, 'Education_teaching': 132, 'Reforming_a_system': 132, 'GetReady': 127, }
% Novel: {'Surrounding': 125, 'Writing': 124, 'Reveal_secret': 124, 'Forming_relationships': 123, 'Hiding_objects': 123, 'Filling': 119, 'Bearing_arms': 117, 'Commerce_pay': 115, 'Kidnapping': 109, 'Patrolling': 108, 'Research': 108, 'Rewards_and_punishments': 106, 'Cost': 104, 'Having_or_lacking_access': 102, 'Adducing': 100, 'Limiting': 96, 'Wearing': 95, 'Cure': 88, 'Create_artwork': 87, 'Exchange': 80, 'Imposing_obligation': 76, 'Award': 71, 'Robbery': 70, 'Containing': 70, 'Prison': 70, 'Commerce_buy': 64, 'Revenge': 64, 'Carry_goods': 62, 'Rite': 59, 'Submitting_documents': 58, 'Practice': 46, 'Lighting': 44, 'Labeling': 43, 'Scouring': 40, 'Justifying': 34, 'Ratification': 33, 'Suspicion': 27, 'Vocalizations': 25, 'Theft': 24, 'Ingestion': 23, 'Renting': 21, 'Incident': 17, 'Institutionalization': 15, 'Risk': 15, 'Extradition': 14}


% \begin{table}[h]
% \centering
% \small
% \begin{tabular}{l|c|c|c}
% \toprule
%     {\textbf{Event Rep}} &  Supervised & Few-shot & Zero-shot \\ 
% \midrule
%     Event type name & &\\
%     Definition &  &\\
%     Seed Trigger & &\\
%     Structure & &\\
% \midrule
%     Majority voting  &  &\\
%     Fusion &   & \\
%     Template &   & & \\
% \bottomrule
% \end{tabular}
% \caption{Performance of trigger extraction on KBP (F1-score, \%)}
% \label{tab:Entity}
% \end{table}
\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{plot.png}
  \vspace{-0.6em}
  \caption{F-score distribution of all novel types based on various event type prompts under the few-shot event detection setting on ACE (Best view in color)}
  \label{fig:f1_distribution}
  \vspace{-1.2em}
\end{figure*}

\section{Results and Discussion}

\paragraph{Overall Results}
The experimental results for supervised, few-shot and zero-shot event detection on ACE05, ERE and MAVEN are shown in Table~\ref{tab:ACE}-\ref{tab:MAVEN}, from which we see that (1) the APEX prompt achieves the best performance among all the forms of prompts under all the settings of the three benchmark datasets. Comparing with the previous state of the art, the APEX prompt shows up to 4\% F-score gain for supervised event detection (on ERE), 22.2\% F-score gain for few-shot event detection (on ACE), and 24.3\% F-score gain for zero-shot event detection (on MAVEN); (2) All the forms of prompts provide significant improvement for few-shot and zero-shot event detection, demonstrating the benefit of leveraging the semantics of event types via various forms of prompts for event detection, especially when the annotations are limited or not available. (3) Continuous soft prompt does not provide comparable performance as other forms of event type representations, which proves the necessity of leveraging event type specific prior knowledge to the representations; (4) The majority voting does not show improvement over individual prompts, due to the fact that each individual prompt captures a particular aspect of the event type semantics.

\paragraph{Supervised Event Detection}
By carefully investigating the event mentions that are correctly detected by the APEX prompt while missed by other prompts, we find that the APEX prompt is more effective in detecting two types of event mentions: homonyms (multiple-meaning words) and intricate words. General homonyms are usually hard to be detected as event mentions as they usually have dozens of meanings in different contexts. For example, consider the following two examples: (i) \textit{Airlines are getting [Transport:Movement] flyers to destinations on time more often .} (ii) \textit{If the board cannot vote to give [Transaction:Transfer-Money'] themselves present money}. Here, ``get'', and ``give'' are not detected based on the event type name or seed triggers but correctly identified by the definition and APEX prompts. In general, the definition and APEX prompts make 10\% and 7\% fewer false predictions than seed triggers on general homonyms. For intricate words, their semantics usually cannot be captured with an individual prompt. In the following two examples: (i) \textit{It is reasonable, however, to reimburse board members for legitimate expenses}
(ii) \textit{$\cdot\cdot\cdot$ ever having discussed being compensated by the board in the future $\cdot\cdot\cdot$}, ``reimburse'' and ``compensated'' indicate sophisticated meaning of \textit{Transaction:Transfer-Money}, which may not be captured by prompts, such as seed triggers. With the event definition and the argument roles in the APEX prompt, the highly correlated contexts, such as ``board members'' and ``legitimate expenses'', can help the model correctly detect \textit{reimburse} as an event mention of \textit{Transaction:Transfer-Money}.
%the highly correlated tentative \textit{Person} argument role of ``board members" and the amount of money to be transferred, ``legitimate expenses", help to detect the target trigger\lifu{re-write this sentence}.


% The experimental results for supervised event trigger extraction are shown in Table \ref{tab:ACE}-\ref{tab:MAVEN}. 
% The experiment results demonstrates that the comprehensive prompt is more effective in detecting event triggers. It outperforms the best individual representation prompt by 1.2 and 3.0 percentage points on ACE and ERE respectively. 

% We investigate trigger candidates that have been labeled differently with different types of prompt,  and found comprehensive APEX prompt more effective in detecting two types of triggers: homonyms (multiple-meaning words) and intricate words.
% % resolving two types of errors that commonly occur compared with seed trigger-based queries \cite{wang2021query}. 
% General homonyms are difficult to be identified as an event trigger, because they usually have dozens of meanings conditioning on the context. For example,  the ``get", and the ``give" in the following examples are not detected with type name or seed trigger prompts: (i) \textit{Airlines are getting [Transport:Movement] flyers to destinations on time more often .}
% (ii) \textit{If the board cannot vote to give [Transaction:Transfer-Money'] themselves present money}. 
% In general, definition-based prompts and comprehensive APEX prompts make 10\% and 7\% fewer false predictions than Seed trigger-based prompts on general homonyms.

% Another type is those intricate words whose semantics cannot be captured with an individual prompt. For example, the ``reimburse" and ``compensated" in the following example contains the sophisticated meaning of \textit{Transaction:Transfer-Money}, which seed triggers might not cover: 
% (i) \textit{It is reasonable, however, to reimburse board members for legitimate expenses}
% (ii) \textit{$\cdot\cdot\cdot$ ever having discussed being compensated by the board in the future $\cdot\cdot\cdot$}
% With the event definition and the argument information in the APEX prompt, the highly correlated tentative \textit{Person} argument role of ``board members" and the amount of money to be transferred, ``legitimate expenses", help to detect the target trigger. 



% Following \cite{honey_chen_2021} \sijia{need rephrase}
% We conducted experiments on ACE05, MAVEN and ERE datasets. 
% We split train/dev/test sets according
% to event types and we use event types with more
% instances for training, the other for dev/test. To
% conduct 5-shot experiments, we filter event types
% less than 6 instances. Finally, for ACE05, its
% train/dev/test set contains 3598/140/149 instances
% and 20/10/10 types respectively, for MAVEN, those
% are 34651/1494/1505 instances and 120/45/45
% types
% The experimental results for few-shot event trigger extraction are shown in Table \ref{tab:ACE}-\ref{tab:ERE}. 
% Event name and seed trigger have better performance than definition and event structure because they are easier to be aligned in the embedding spaces. The comprehensive prompt that includes the definition and structure striking outperforms individual type name or seed trigger, proving the effectiveness of including them in the prompt.


\paragraph{Few-shot Event Detection}
Figure~\ref{fig:f1_distribution} shows the F-score distribution of all novel types based on various forms of event type prompts, from which we observe that:
(1) The event type name, seed triggers, and APEX prompt generally perform better than definition and structure, as they carry more straightforward semantics of event types. (2) Event type name based prompts show lower performance on \textit{Personnel:End-Position}, \textit{Personnel:Start-Position} and \textit{Transaction:Transfer-Money} than other event types, as the semantics of these event type names are less indicative than other event types. (3) Seed triggers based prompts perform worse than event type name and APEX prompts on two event types, \textit{Life:injure} and \textit{Life:die}, probably because the prototype seed triggers are not properly selected. (4) The structure based prompt outperforms the other prompts on \textit{Life:Injure} as \textit{Life:Injure} events require the existence of a person or victim. (5) APEX prompt shows consistently (almost) best performance on all the event types, due to the fact that it combines all the information of other prompts. (6) We also observe that the performance of \textit{Life:Be-Born}, \textit{Life:Die}, \textit{Life:Marry}, and \textit{Personnel:Elect} based on various forms of prompts are consistently better than the other types as the intrinsic semantics of those types the corresponding event triggers are concentrated. 


\paragraph{Zero-shot Event Detection} The proposed prompt-based method is more affordable to be generalized comparing with the prior state-of-the-art approach~\cite{zhang-etal-2021-zero}. The average length of created APEX prompts is less than 20 tokens, thus manually creating them won't take much human effort. On the contrary,~\newcite{zhang-etal-2021-zero} requires a large collection of anchor sentences to perform zero-shot event detection, e.g., 4,556,237 anchor sentences for ACE and ERE. This process is time consuming and expensive.
%since the performance achieved by The benchmark model~\cite{zhang-etal-2021-zero} on ACE and ERE depends on the 4,556,237 collected anchor sentences, to achieve decent performance on MAVEN, they need to collect larger scale anchor sentences. This process is time consuming and expensive.\lifu{rewrite this paragraph}
% The benchmark model\cite{zhang-etal-2021-zero} collects 4,556,237 anchor sentences during the pre-process stage, which is  difficult and time-consuming. Though such prior knowledge have been proven to be effective for ACE and ERE, the prior knowledge is difficult to generalize to other ontologies.  To better detect MAVEN events, they either need to collect larger scale anchor sentences or design a more sophisticated collection protocol.\lifu{rewrite this paragraph}

% The experimental results for zero-shot event trigger extraction are shown in Table \ref{tab:ACE}-\ref{tab:ERE}. The results demonstrate that the comprehensive prompt is the most effect event type representation, especially for ACE (with 2.9 percentage points performance gain in F1 score) and MAVEN (2.3 percentage points gain).

% The proposed prompt-based method is also more affordable to generalize compared to the benchmark model in \cite{zhang-etal-2021-zero}. The average length of created comprehensive prompts is less than 20 tokens. 
% The benchmark model\cite{zhang-etal-2021-zero} collects 4,556,237 anchor sentences during the pre-process stage, which is  difficult and time-consuming. Though such prior knowledge have been proven to be effective for ACE and ERE, the prior knowledge is difficult to generalize to other ontologies.  To better detect MAVEN events, they either need to collect larger scale anchor sentences or design a more sophisticated collection protocol.



% \paragraph{Ablation Study}
% We first compare with event type representation assemble strategy, majority voting with our proposed comprehensive template. Taking the majority of predictions can theoretically improve the confidence in predication. Nevertheless, our experimental result shows that this strategy can only improve the performance when each model perform well. If the models have large performance gap, then taking the majority of predictions might not outperform the model trained with best event type representation.


% In addition to discrete prompt, we also investigate soft prompt. Instead of the discrete prompt tokens, we assign fixed-length trainable continuous vectors for each event type specific query and label the input sentence accordingly.
% Soft prompt does not apply for zero-shot learning because the continuous vector is meaningless unless trained with annotated data. Therefore we conducted experiments under supervised learning and few-shot leaning settings.
% \sijia{(1) add a prompt that is based on event type specific question; (2) try p-tuning + sequence labeling for supervised event extraction}


\paragraph{Remaining Challenges} We have demonstrated that a proper description can provide much better performance for both supervised and weakly supervised event detection. However, the event types from most existing ontologies are not properly defined. For example, in ACE annotation guideline~\cite{ldc_ace05}, \textit{transfer-money} is defined as ``\textit{giving, receiving, borrowing, or lending money when it is not in the context of purchasing something}'', however, it's hard for the model to accurately interpret it, especially the constraints ``\textit{not in the context of purchasing something}''. 
%descriptions are not clear enough. Many event types in ACE and ERE are not properly defined with a clear description in the annotation guidelines~\cite{ldc_ace05, song2015light}, 
% \sijia{e.g. subtypes in \textit{Contact} event main type are determined by annotated attributes, and \textit{Contact.Contact} event occurs when the medium or audience is not explicitly stated. }
%\sijia{Manufacture:Artifact is a new event type in ERE without proper definition.}
%\lifu{we are saying the definitions are not always clear, we need to show an example to prove that} 
In addition, many event types from MAVEN, e.g., \textit{Achieve}, \textit{Award}, and \textit{Incident}, are not associated with any definitions. 
%Most event types in MAVEN are adapted from FrameNet~\cite{baker1998berkeley}, where event types are described in natural languages. However, there are still some types that are not well defined, e.g., \textit{Achieve}, \textit{Award}, and \textit{Incident}. 
A potential future research direction is to leverage mining-based approaches or state-of-the-art generators to automatically generate a comprehensive event type description based on various sources, such as annotation guidelines, example annotations, and external knowledge bases.

% Lack of proper definition is a potential challenge for future ontologies. The event types in ACE and ERE are explicitly defined \cite{ldc_ace05}; however, it is not always true. Most event types in MAVEN are adapted from FrameNet, where event types are defined in natural languages; however, the rest are not, leaving them undefined. 
% A potential future approach is to automatically summarize the event definitions or build a prior knowledge base for event types, either from external resources or training data. \lifu{expand this paragraph and add more, e.g., how to automatically select the best prompt, or generate the prompt}
% prompt mining
% Prompt Paraphrasing and Prompt Generation
% Hard-Soft Prompt Hybrid Tuning
%\sijia{Mining-based approaches can automatically find templates from a large text corpus such as Wikipedia. Prompts can be generated using standard natural language generation models, or paraphrased from the proposed comprehensive prompt. Additionally, instead of purely discrete or soft prompt, combining actual tokens and virtual tokens could leverage both the prior knowledge created manually and the learning flexibility of soft prompt.}

% \sijia{}
% In this section, we will discuss some remaining challenges with examples.
% The first common mistake is on hypothetical or negative events, that is, hypothetical or believed to happen but not. For example, in the following two examples, our model predict \textit{casualties} and \textit{acquire} as \textit{Life:Die-Person} and \textit{Transaction:Transfer-Ownership}, but they are not true event triggers: 
% \textit{(i) There was no clear figure of Iraqi casualties[Pred: Life:Die-Person]. 
% (ii) American International Group Inc. is likely to acquire[Pred: Transaction:Transfer-Ownership] all shares.}



% Furthermore, the discrete comprehensive prompt is manually designed, thus the searching space is discrete and hard to optimize. Though the event type name and seed triggers in the comprehensive template prompt can be automatically or statistically formulated, we manually combine the definition and event arguments. 


==> Event Detection based on Type Specific Prompts/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We investigate a variety of prompts to represent the semantics of event types, and leverage them with a unified framework for supervised, few-shot and zero-shot event detection. Experimental results demonstrate that, a well-defined and comprehensive description of event types can significantly improve the performance of event detection, especially when the annotations are limited (few-shot event detection) or even not available (zero-shot event detection), with up to 24.3\% F-score gain over the prior state of the art. In the future, we will explore mining-based or generation-based approaches to automatically generate a comprehensive description of each event type from available resources and external knowledge base.

%To evaluate the effect of prompt design in detecting event triggers, this paper investigate various forms of event type specific prompts, and conducted extensive experiments under three different settings, supervised learning, few-shot and zero-shot learning. Experimental results demonstrate the effectiveness of a well-defined prompt in improving the event detection performance, especially when the learning data is scarce. 
% This work illustrate related aspects that can be leveraged to design finer prompt. We pointed out a  
